Radio Resource Management for V2V Multihop Communication Considering Adjacent Channel Interference

This paper investigate joint scheduling and power control for V2V multicast allowing multihop communication. The effects of both co-channel interference and adjacent channel interference are considered. First, we solve the problem with the objective of maximizing the throughput and connectivity of vehicles in the network. Then extend the same problem formulation to include the objective of minimizing the latency and the average age of information (AoI), which is the age of the latest received message. In order to account for fairness, we also show the problem formulation to maximize the worst-case throughput and connectivity. All the problems are formulated as mixed Boolean linear programming problems, which allows computation of optimal solutions. Furthermore, we consider the error probability of a link failure in all the problem formulations and accommodate the probability requirements for satisfying a certain throughput/connectivity/latency/AoI. In order to support a large V2V network, a clustering algorithm is proposed whose computational complexity scale well with the network size. To handle the case of zero channel information at the scheduler, a multihop distributed scheduling scheme is proposed.

==> Drawings/acir.tex <==
%% ACIR Drawing
\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}
\tikzstyle{gArea} = [pattern=north west lines, draw=green,pattern color=green]
\tikzstyle{rArea} = [pattern=north east lines, draw=red,pattern color=red]
\tikzstyle{lStyle} = [dash dot,thick,black!50]
\begin{tikzpicture}
%% Transmitter
%\draw[thick,->] (-.25,0) -- (7,0) node[below]{Frequency};
%\draw[thick,->] (0,-.25) -- (0,3.5);
%\node[anchor=west,rotate=90] at (-.2cm,0.1) {Tx Power (dBm/Hz)};
%\begin{pgfonlayer}{bg}
%\draw[gArea] (1.5,0) {[rounded corners] -- ++(0.1,2)  --  node[anchor=south]{Transmitter $i$} ++(1,0)} -- ++(0.1,-2) -- cycle;
%\draw[rArea,xshift=4cm] (0,0) {[rounded corners] -- ++(0.2,3)  -- node[anchor=south]{Transmitter $k$} ++(1,0)} -- ++(0.2,-3) -- cycle;
%\end{pgfonlayer}
% Receiver
\begin{scope}[yshift=-4cm,scale = 1.2]{Receiver}
\draw[thick,->] (-.25,0) -- (7,0) node[anchor=north east]{Frequency};
\draw[thick,->] (0,-.25) -- (0,3.5);
\node[anchor=west,rotate=90] at (-.2cm,0.1) {Rx Power (dBm/Hz)};
\begin{pgfonlayer}{bg}
\draw[gArea] (.2,0) {[rounded corners] -- ++(30:1.5) -- ++(0.1,1) -- node(A){} ++(1,0) --++(0.1,-1) -- ++(-30:1.5)} -- cycle;
\draw[rArea,xshift=4cm] (-3.3,0)  {[rounded corners] -- ++(30:3.8) -- ++(0.2,1) -- node(B){} ++(1,0) --++(0.2,-1)}  {[opacity=0]  -- ++(-30:1) -- ++(0,-1.38)} -- cycle;
\end{pgfonlayer}
% ACIR marking
%\draw[lStyle,dash phase=25pt] (A) -- node[above=0.3,black]{Receiver $j$} ++(-3.6cm,0) node(Ae){};
\draw[lStyle,dash phase=40pt] (B) --  ++(-3.6cm,0) node(Bl){};
\draw[lStyle] ($(A)+(4.5,-.8)$) node(Adr){}  -- ++(-5.5cm,0) node(Al){};
\draw[<->,thick,black!50] ($(Bl)+(0.2,-1pt)$) -- node[left,black]{ACIR} ++(0,-1.9);

\draw[lStyle,dash phase=13pt] ($(A)$)  -- ++(4.5cm,0) node(Ar){};
\draw[<->,thick,black!50] ($(Ar)+(-.1,-.05)$) -- node[right,black]{$\mathrm{SIR}_{i,j}$} ++(0,-.7);

\node[above,text width=2cm, align=center]  at ($(A)+(0,1.2)$) {Received signal from transmitter $i$};
\node[above,text width=2cm, align=center]  at ($(B)+(0,0)$) {Received signal from transmitter $k$};
\end{scope}
\end{tikzpicture}

==> Paper 3_ Multihop communication with ACI/Drawings/acir.tex <==
%% ACIR Drawing
\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}
\tikzstyle{gArea} = [pattern=north west lines, draw=green,pattern color=green]
\tikzstyle{rArea} = [pattern=north east lines, draw=red,pattern color=red]
\tikzstyle{lStyle} = [dash dot,thick,black!50]
\begin{tikzpicture}
%% Transmitter
%\draw[thick,->] (-.25,0) -- (7,0) node[below]{Frequency};
%\draw[thick,->] (0,-.25) -- (0,3.5);
%\node[anchor=west,rotate=90] at (-.2cm,0.1) {Tx Power (dBm/Hz)};
%\begin{pgfonlayer}{bg}
%\draw[gArea] (1.5,0) {[rounded corners] -- ++(0.1,2)  --  node[anchor=south]{Transmitter $i$} ++(1,0)} -- ++(0.1,-2) -- cycle;
%\draw[rArea,xshift=4cm] (0,0) {[rounded corners] -- ++(0.2,3)  -- node[anchor=south]{Transmitter $k$} ++(1,0)} -- ++(0.2,-3) -- cycle;
%\end{pgfonlayer}
% Receiver
\begin{scope}[yshift=-4cm,scale = 1.2]{Receiver}
\draw[thick,->] (-.25,0) -- (7,0) node[anchor=north east]{Frequency};
\draw[thick,->] (0,-.25) -- (0,3.5);
\node[anchor=west,rotate=90] at (-.2cm,0.1) {Rx Power (dBm/Hz)};
\begin{pgfonlayer}{bg}
\draw[gArea] (.2,0) {[rounded corners] -- ++(30:1.5) -- ++(0.1,1) -- node(A){} ++(1,0) --++(0.1,-1) -- ++(-30:1.5)} -- cycle;
\draw[rArea,xshift=4cm] (-3.3,0)  {[rounded corners] -- ++(30:3.8) -- ++(0.2,1) -- node(B){} ++(1,0) --++(0.2,-1)}  {[opacity=0]  -- ++(-30:1) -- ++(0,-1.38)} -- cycle;
\end{pgfonlayer}
% ACIR marking
%\draw[lStyle,dash phase=25pt] (A) -- node[above=0.3,black]{Receiver $j$} ++(-3.6cm,0) node(Ae){};
\draw[lStyle,dash phase=40pt] (B) --  ++(-3.6cm,0) node(Bl){};
\draw[lStyle] ($(A)+(4.5,-.8)$) node(Adr){}  -- ++(-5.5cm,0) node(Al){};
\draw[<->,thick,black!50] ($(Bl)+(0.2,-1pt)$) -- node[left,black]{ACIR} ++(0,-1.9);

\draw[lStyle,dash phase=13pt] ($(A)$)  -- ++(4.5cm,0) node(Ar){};
\draw[<->,thick,black!50] ($(Ar)+(-.1,-.05)$) -- node[right,black]{$\mathrm{SIR}_{i,j}$} ++(0,-.7);

\node[above,text width=2cm, align=center]  at ($(A)+(0,1.2)$) {Received signal from transmitter $i$};
\node[above,text width=2cm, align=center]  at ($(B)+(0,0)$) {Received signal from transmitter $k$};
\end{scope}
\end{tikzpicture}

==> Paper 3_ Multihop communication with ACI/Drawings/acir_lambda.tex <==

%% ACIR Drawing
\tikzstyle{rArea} = [pattern=north east lines, draw=red,pattern color=red]
\tikzstyle{lStyle} = [dash dot,thick,black!50]


\begin{tikzpicture}
% Receiver
\begin{scope}[yshift=-4cm,scale = 1.2]{Receiver}

%% Draw axes
\draw[thick,->] (-.25,0) -- (5.5,0) node[anchor=north east]{Frequency slots};
\draw[thick,->] (0,-.25) -- (0,1.3);
\node[anchor=west,rotate=90] at (-.2cm,-0) {Rx Power};

%% Draw ACI, i.e., red area
\draw[rArea,xshift=0cm] (0,0) -- (0,0.3)  {[rounded corners] -- ++(20:1) -- ++(0.2,0.6) node(fp1){} --  ++(0.7,0) node(fp2){} --  ++(0.2,-0.6)}  --node(f1){} ++(-20:1.9);

%% Mark f'
\draw[lStyle,dash phase=40pt] (fp1) --  ++(0,-1.4) node[xshift=0.5cm,yshift=-0.1cm,black](){$f'$};
\draw[lStyle,dash phase=40pt] (fp2) --  ++(0,-1.4);

%% Mark f
\draw[lStyle,dash phase=40pt] ($(f1)+(-0.3,0.1)$) node(f1new){} --  ++(0,-0.6) node[xshift=0.35cm,yshift=-0.1cm,black](){$f$};
\draw[lStyle,dash phase=40pt] ($(f1new)+(0.65,-0.3)$) --  ++(0,-0.25);

%% Mark \lambda
\draw[lStyle,dash phase=40pt] (fp1) --  ++(2.8,0) node(lambdaTop){};
\draw[lStyle,dash phase=40pt] ($(f1new)+(0.2,-0.1)$) --  ++(1.1,0) node(lambdaBottom){};
\draw[lStyle,dash phase=40pt,<->] (lambdaTop) -- node[xshift=1.1cm, black](){$-\lambda_{|f'-f|}$(dB)} (lambdaBottom);

\end{scope}
\end{tikzpicture}

==> Paper 3_ Multihop communication with ACI/Drawings/carsOnStreet.tex <==
\newcommand{\scaleValueOfCar}{0.1}
\begin{tikzpicture}[
%% -Draw Car
carDrawing/.pic={ 
	\draw[scale=\scaleValueOfCar,color=black,very thin] (1.5,.5) -- ++(0,1.3) -- ++(1,0) --  ++(3,0) -- ++(1,-0.3) -- ++(0,-1) -- (1.5,.5) -- cycle;    	%% Bottom body, with "bottom left point" as starting point
	\draw[scale=\scaleValueOfCar,rounded corners=0.05ex,fill=white,very thin]  (2,1.8) -- ++(0.5,0.7) -- ++(1.8,0) -- ++(0.8,-0.7) -- cycle;			  %% Top body, with "bottom left point" as starting point
	\draw[scale=\scaleValueOfCar,very thin]  (3.7,1.8) -- (3.7,2.5);
	\draw[scale=\scaleValueOfCar,draw=black,fill=white!50,very thin] (2.75,.5) circle (.5);	%% white instead of gray
	\draw[scale=\scaleValueOfCar,draw=black,fill=white!50,very thin] (5.5,.5) circle (.5);
	\draw[scale=\scaleValueOfCar,draw=black,fill=white!80,very thin] (2.75,.5) circle (.4);
	\draw[scale=\scaleValueOfCar,draw=black,fill=white!80,very thin] (5.5,.5) circle (.4);
}]

%% Road lines
\draw[line width=0.1,color=black!50] (0,0.5cm)--(16cm,0.5cm);
\draw[line width=0.1,dashed,color=black!50] (0,0)--(16cm,0);
\draw[line width=0.1,color=black!50] (0,-0.5cm)--(16cm,-0.5cm);

%\draw[-LaTeX, line width=.0.5cm] (.5,-1) --++(3,0) node[pos=.2, above] {Car lane};
%\draw[-LaTeX, line width=.0.5cm, red] (.5,1)  --++(3,0) node[pos=.2, above] {Bus lane};


%% -Cluster c, c+1
%  Top line of road
\draw (1cm,0.1cm) node(VUEi){} pic[] {carDrawing};   
\draw (2cm,0.1cm) pic[] {carDrawing};  %% Cluster 'c' center here
\draw (3.8cm,0.1cm) node(VUEj){} pic[] {carDrawing};   
\draw (4.8cm,0.1cm) pic[] {carDrawing}; 
\draw (5.8cm,0.1cm) pic[] {carDrawing};   
\draw (6.5cm,0.1cm) pic[] {carDrawing}; %% Cluster 'c+1' center here
\draw (7.5cm,0.1cm) pic[] {carDrawing};   

\draw (8.5cm,0.1cm) pic[] {carDrawing};   
\draw (9.3cm,0.1cm) pic[] {carDrawing}; 
\draw (10.1cm,0.1cm) pic[] {carDrawing};   
\draw (11.1cm,0.1cm) pic[] {carDrawing}; 
\draw (11.9cm,0.1cm) pic[] {carDrawing};   
\draw (13cm,0.1cm) pic[] {carDrawing};
\draw (13.9cm,0.1cm) pic[] {carDrawing};   
\draw (15cm,0.1cm) pic[] {carDrawing};   

%  Bottom line of road
\draw (0.3cm,-0.4cm) pic[] {carDrawing};   
\draw (1.2cm,-0.4cm) pic[] {carDrawing};   
%\draw (1.9cm,-0.4cm) pic[] {carDrawing};   
\draw (3cm,-0.3cm) node(VUEkA){} pic[] {carDrawing};   
\draw (3.9cm,-0.4cm) pic[] {carDrawing};   
\draw (5.7cm,-0.4cm) pic[] {carDrawing};   
\draw (6.6cm,-0.4cm) pic[] {carDrawing};   
\draw (7.5cm,-0.4cm) pic[] {carDrawing};   

\draw (8.7cm,-0.4cm) pic[] {carDrawing};   
\draw (9.4cm,-0.4cm) pic[] {carDrawing}; 
\draw (10.4cm,-0.4cm) pic[] {carDrawing};   
\draw (11.9cm,-0.4cm) pic[] {carDrawing}; 
\draw (12.9cm,-0.4cm) pic[] {carDrawing};   
\draw (13.9cm,-0.4cm) pic[] {carDrawing};
\draw (15.1cm,-0.4cm) pic[] {carDrawing};   


%% -VUE i, j, k1 labeling
\draw[->,black]  ($(VUEi)+(-0.3cm,-1cm)$) node[black,below,xshift=-0.1cm]{VUE\,$i$} -- ($(VUEi)+(0.2cm,0cm)$);
%\draw[->,black]  ($(VUEkA)+(0.2cm,-0.6cm)$) node[black,below,xshift=0.1cm]{VUE\,$k_1$} -- ($(VUEkA)+(0.4cm,0cm)$);
\draw[->,black]  ($(VUEkA)+(0.2cm,-0.6cm)$) node[black,below,xshift=0.1cm]{VUE\,$j$} -- ($(VUEkA)+(0.4cm,0cm)$);
%\draw[->,black]  ($(VUEj)+(1.4cm,-1cm)$) node[black,below,xshift=0.2cm]{VUE\,$j$} -- ($(VUEj)+(0.6cm,0cm)$);

%% -Green Cluster drawing and labeling,
\coordinate (cluster1center) at (1.9cm,0cm);
\node[above,xshift=-0.1cm,yshift=1.2cm] at (cluster1center) {Group\,$(c,g)$};
\draw[color=green!50!black]  (cluster1center) ellipse (1cm and 0.5cm);
%\draw[color=green!50!black,dashed]  ($(cluster1center)+(0.5cm,0cm)$) ellipse (2.3cm and 0.7cm);
\draw[color=green!50!black,dashed]  (cluster1center) ellipse (2cm and 0.7cm);

\draw[->] ($(cluster1center)+(-1.1cm,0.7cm)$) node[above,xshift=0.1cm]{$\Ts^{(c,g)}$} -- ($(cluster1center)+(-0.8cm,0.3cm)$);
\draw[->] ($(cluster1center)+(-2.1cm,0.7cm)$) node[above,xshift=0.1cm]{$\Rs^{(c,g)}$} -- ($(cluster1center)+(-1.8cm,0.3cm)$);

%% -Blue Cluster drawing and labeling,
\coordinate (cluster1center) at (3.9cm,0cm);
\node[above,xshift=0.5cm,yshift=1.2cm] at (cluster1center) {Group\,$(c,g+1)$};
\draw[color=blue]  (cluster1center) ellipse (1cm and 0.5cm);
\draw[color=blue,dashed]  (cluster1center) ellipse (2cm and 0.7cm);

\draw[->] ($(cluster1center)+(1.1cm,0.7cm)$) node[above,xshift=0.1cm]{$\Ts^{(c,g+1)}$} -- ($(cluster1center)+(0.8cm,0.3cm)$);
\draw[->] ($(cluster1center)+(2.1cm,0.7cm)$) node[above,xshift=0.5cm]{$\Rs^{(c,g+1)}$} -- ($(cluster1center)+(1.8cm,0.3cm)$);

%% -Red Cluster drawing and labeling,
\coordinate (cluster2center) at (12cm,0cm);
\node[above,yshift=1.2cm] at (cluster2center) {Group\,$(c+1,g)$};
\draw[color=red] (cluster2center) ellipse (1cm and 0.5cm);
\draw[color=red,dashed]  (cluster2center) ellipse (2cm and 0.7cm);

\draw[->] ($(cluster2center)+(-1.1cm,0.7cm)$) node[above,xshift=0.5cm]{$\Ts^{(c+1,g)}$} -- ($(cluster2center)+(-0.8cm,0.3cm)$);
\draw[->] ($(cluster2center)+(-2cm,0.7cm)$) node[above,xshift=0.1cm]{$\Rs^{(c+1,g)}$} -- ($(cluster2center)+(-1.8cm,0.3cm)$);

\end{tikzpicture}

==> Paper 3_ Multihop communication with ACI/Drawings/vueDropping.tex <==



%% VUE Dropping Drawing
\begin{tikzpicture}[rec/.style={rounded corners,inner sep=10pt,draw}]
\node(VUEi) at (0,0) [rec]{VUE $i$} ;
\node(VUEj) at (4,0) [rec]{VUE $j$} ;
\node(VUEk) at (7,0) [rec]{VUE $k$} ;
%\draw[thick,dash dot] ($(VUEi.east)+(5pt,0)$) -- ($(VUEj.west)-(5pt,0)$);
%\draw[thick,dash dot] ($(VUEj.east)+(5pt,0)$) -- ($(VUEk.west)-(5pt,0)$);
\draw[bend left,->,color=green] (VUEi) to node[above,black]{Desired link} (VUEj);
\draw[bend right,->,color=red,thick] (VUEk) to node[above,black]{Interference link} (VUEj);
\draw[bend left,->,color=green] (VUEi) to node[below,black]{$H_{i,j}$} (VUEj);
%\draw[bend right,->,color=red,thick] (VUEk) to node[below,black]{$G^t_{k,i,j}$} (VUEj);		%% Printing of G^t_{k,i,j}
\end{tikzpicture}




==> Paper 3_ Multihop communication with ACI/Plots/plot_performance1.tex <==
%\pgfplotstableread[col sep=comma,]{\folderName/schPerformanceForEqualPower.csv}\datatable1

\newcommand{\folderName}{Plots}

\pgfplotscreateplotcyclelist{colorList1}{
	{black,mark=+},
	{violet,mark=square,mark options={fill=none}},
	{green,mark=triangle},
	{blue,mark=o},
	{red,mark=star},
}

\begingroup
\thickmuskip=0mu		%% To reduce space around '='

\begin{figure*}[!ht] 	
	\centering	
	
	\begin{tikzpicture}
	\begin{groupplot}[cycle list name=colorList1, xmajorgrids, ymajorgrids,
	group style={group name=my plots,group size= 3 by 1,vertical sep=2.5cm },
	height=5cm,width=0.3\paperwidth	%%0.735\columnwidth
	]
	
	
	%% 1st Plot   xAxis = T
	\nextgroupplot[
	%xmin=1, xmax=5,
	%ymin=0,ymax=6,
	xlabel=$\nTx$,
	xtick =  {10, 20, 30, 40, 50} %\plotAxTicklabels,
	]
	\addplot +[restrict expr to domain={\coordindex}{0:9}]   table [x=xValues, y=sch_Peng1, col sep=comma] {\folderName/nSuccessfullLinks_nTx.csv}; \label{figA:plot1} 
	\addplot +[restrict expr to domain={\coordindex}{0:9}]   table [x=xValues, y=sch_Heuristic1, col sep=comma] {\folderName/nSuccessfullLinks_nTx.csv}; \label{figA:plot2} 
	\addplot +[restrict expr to domain={\coordindex}{0:9}]   table [x=xValues, y=DCS, col sep=comma] {\folderName/nSuccessfullLinks_nTx.csv}; \label{figA:plot3} 
	\addplot +[restrict expr to domain={\coordindex}{0:9}]   table [x=xValues, y=joint_noMultihop, col sep=comma] {\folderName/nSuccessfullLinks_nTx.csv}; \label{figA:plot4} 
	\addplot +[restrict expr to domain={\coordindex}{0:9}]   table [x=xValues, y=joint_basic2, col sep=comma] {\folderName/nSuccessfullLinks_nTx.csv}; \label{figA:plot5} 
	
	%% 2nd Plot  xAxis = F
	\nextgroupplot[
	%xmin=6, xmax=20,
	%ymin=0,ymax=15,
	xlabel=$T$,
	xtick =  {4,8,12,16},
	legend style={at={(0.5,1.08)},anchor=south, legend columns=-1, column sep = 0.1cm}, % col sep=-0.1cm
	]
	%\addplot  table [x=xValues, y=sch_Heuristic1, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv}; \addlegendentry{\hspace{-0.1cm} Heuristic scheduling \em}
	%\addplot  table [x=xValues, y=DCS, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv};\addlegendentry{\hspace{-0.1cm} Optimal scheduling \em}
	%\addplot  table [x=xValues, y=joint_noMultihop, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv};\addlegendentry{\hspace{-0.1cm} Joint scheduling and power control (column generation) \em}
	%\addplot  table [x=xValues, y=joint_basic2, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv};\addlegendentry{\hspace{-0.1cm} Joint scheduling and power control (near-optimal) \em}
	\addplot  table [x=xValues, y=sch_Peng1, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv}; 
	\addplot  table [x=xValues, y=sch_Heuristic1, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv}; 
	\addplot  table [x=xValues, y=DCS, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv};
	\addplot  table [x=xValues, y=joint_noMultihop, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv};
	\addplot  table [x=xValues, y=joint_basic2, col sep=comma] {\folderName/nSuccessfullLinks_omega.csv};
	\coordinate (top) at (rel axis cs:0,1);% coordinate at top of the first plot
	
	%% 3rd Plot   xAxis = N
	\nextgroupplot[
	%xmin=5, xmax=25,
	%ymin=0,ymax=5,
	xlabel=$\nRx$,
	xtick =  {4,8,12,16,20},
	]
	\addplot  table [x=xValues, y=sch_Peng1, col sep=comma] {\folderName/nSuccessfullLinks_nRx.csv};
	\addplot  table [x=xValues, y=sch_Heuristic1, col sep=comma] {\folderName/nSuccessfullLinks_nRx.csv};
	\addplot  table [x=xValues, y=DCS, col sep=comma] {\folderName/nSuccessfullLinks_nRx.csv};
	\addplot  table [x=xValues, y=joint_noMultihop, col sep=comma] {\folderName/nSuccessfullLinks_nRx.csv};
	\addplot  table [x=xValues, y=joint_basic2, col sep=comma] {\folderName/nSuccessfullLinks_nRx.csv};
	
	
	
	%\coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
	\coordinate[right=-5.7cm] (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
	\end{groupplot}
	%% -Captions
	\node[below = 1cm of my plots c1r1.south] {(a) ($T=12,\,\nRx=20$)};
	\node[below = 1cm of my plots c2r1.south] {(b) ($\nTx=20,\,\nRx=20$)};
	\node[below = 1cm of my plots c3r1.south] {(c) ($\nTx=20,\,T=12$)};
	
	
	%% -Legend
	\path (top-|current bounding box.west)--
	node[anchor=south,rotate=90] {\parbox{4.5cm}{\centering Average connectivity of a VUE}}
	(bot-|current bounding box.west);
	\path[yshift=2cm] (top|-current bounding box.north)--
	coordinate(legendpos)
	(bot|-current bounding box.north);
	\matrix[
	matrix of nodes,
	anchor=south,
	draw,
	inner sep=0.2em,
	draw
	]at([yshift=1ex]legendpos)
	{
		\ref{figA:plot5} \eqref{formulation:maximizeConnectivity}  ~~
		\ref{figA:plot4} \eqref{formulation:maximizeConnectivity} without multihop  ~~
		\ref{figA:plot3} CDS (Alg. \ref{Alg:CDS}) \\
		\ref{figA:plot2} Heuristic scheduling  \cite{Anver_Access1} ~~~
		\ref{figA:plot1} \cite{Peng1} \\};
	\end{tikzpicture}
	
	
	\caption{Average connectivity of a VUE for various algorithms} \label{Fig:nSuccessfullLinks}
\end{figure*}

\endgroup

%%%%%%%%%%%%%%%%% FAIRNESS PLOT

%\pgfplotstableread[col sep=comma,]{\folderName/schPerformanceForEqualPower.csv}\datatable1


%\pgfplotscreateplotcyclelist{colorList1}{
%	{black,mark=+},
%	{violet,mark=square,mark options={fill=none}},
%	{green,mark=triangle},
%	{blue,mark=o},
%	{magenta,mark=diamond},
%	{red,mark=star},
%}

\begingroup
\thickmuskip=0mu		%% To reduce space around '='

\begin{figure*}[!ht]	
	\centering	
	
	\begin{tikzpicture}
	\begin{groupplot}[cycle list name=colorList1, xmajorgrids, ymajorgrids,
	group style={group name=my plots,group size= 2 by 1,vertical sep=2.5cm ,horizontal sep=2cm },
	height=5.5cm,width=0.4\paperwidth	%%0.735\columnwidth
	]
	
	
	%% 1st Plot  CDF Plot
	\nextgroupplot[
	%xmin = 0, xmax = 9,
	xtick =  {0,2,4,6,8,10,12,14,16,18,20},			
	xlabel=\parbox{4cm}{\centering Connectivity of a VUE},
	ylabel=CDF,
	%xtick =  {0,1,2,3,4,5,6,7,8,9},
	ymax = 1,
	]
	\addplot table [x=xValues, y=sch_Peng1, col sep=comma] {\folderName/CDF_of_nSuccessfullLinks.csv}; \label{figB:plot1} 
	\addplot table [x=xValues, y=sch_Heuristic1, col sep=comma] {\folderName/CDF_of_nSuccessfullLinks.csv}; \label{figB:plot2} 
	\addplot table [x=xValues, y=DCS, col sep=comma] {\folderName/CDF_of_nSuccessfullLinks.csv}; \label{figB:plot3} 
	\addplot table [x=xValues, y=joint_noMultihop, col sep=comma] {\folderName/CDF_of_nSuccessfullLinks.csv}; \label{figB:plot4} 
	\addplot table [x=xValues, y=joint_basic2, col sep=comma] {\folderName/CDF_of_nSuccessfullLinks.csv}; \label{figB:plot5} 
	
	%% 2nd Plot: #Successful links Vs VUE-index,
	\nextgroupplot[
	xmin = 0, xmax = 19,
	%ymax = 5,  
	xlabel=VUE index ($i$) in a group,	
	ylabel=\parbox{4cm}{\centering Average number of successful links for a VUE ($\bar{Z}_i$) },
	legend style={at={(-0.15,1.08)},anchor=south, legend columns=-1, column sep = 0.1cm}, % col sep=0.2cm
	]
	\addplot table [x=xValues, y=sch_Peng1, col sep=comma] {\folderName/eachVUE_nSuccessfullLinks.csv};
	\addplot table [x=xValues, y=sch_Heuristic1, col sep=comma] {\folderName/eachVUE_nSuccessfullLinks.csv};
	\addplot table [x=xValues, y=DCS, col sep=comma] {\folderName/eachVUE_nSuccessfullLinks.csv};
	\addplot table [x=xValues, y=joint_noMultihop, col sep=comma] {\folderName/eachVUE_nSuccessfullLinks.csv};
	\addplot table [x=xValues, y=joint_basic2, col sep=comma] {\folderName/eachVUE_nSuccessfullLinks.csv};
	
	
	
	%\addplot  table [x=xValues, y=powerControl_equalPower, col sep=comma] {\folderName/powerValuesForNaturalScheduling_F.csv}; \addlegendentry{\hspace{0.2cm}Equal power \em}
	%\addplot  table [x=xValues, y=powerControl_kangWang, col sep=comma] {\folderName/powerValuesForNaturalScheduling_F.csv};\addlegendentry{\hspace{0.2cm}Heuristic power \em}
	%\addplot  table [x=xValues, y=powerControl_gurobi, col sep=comma] {\folderName/powerValuesForNaturalScheduling_F.csv};\addlegendentry{\hspace{0.2cm}Near-optimal power \em}
	%
	%%%% 3rd Plot
	%%\nextgroupplot[
	%%xlabel=$N$,
	%%ymax = 25,
	%%]
	%%\addplot  table [x=xValues, y=powerControl_equalPower, col sep=comma] {\folderName/powerValuesForNaturalScheduling_N.csv};
	%%\addplot  table [x=xValues, y=powerControl_kangWang, col sep=comma] {\folderName/powerValuesForNaturalScheduling_N.csv};
	%%\addplot  table [x=xValues, y=powerControl_gurobi, col sep=comma] {\folderName/powerValuesForNaturalScheduling_N.csv};
	%%
	%%
	
	\coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
	\end{groupplot}
	%% -Captions
	\node[below = 1.3cm of my plots c1r1.south] {(a)};
	\node[below = 1.3cm of my plots c2r1.south] {(b)};
	
	
	%%% -Legend
	%\path (top-|current bounding box.west)--
	%node[anchor=south,rotate=90] {}
	%(bot-|current bounding box.west);
	%\path[yshift=2cm] (top|-current bounding box.north)--
	%coordinate(legendpos)
	%(bot|-current bounding box.north);
	%\matrix[
	%matrix of nodes,
	%anchor=south,
	%draw,
	%inner sep=0.2em,
	%draw
	%]at([yshift=1ex]legendpos)
	%{
	%	\ref{figB:plot2} \em Heuristic scheduling  ~~~
	%	\ref{figB:plot3}\em Optimal scheduling ~~~  \\
	%	\ref{figB:plot4}\em Joint scheduling and power control (column generation) ~~~
	%	\ref{figB:plot5}\em Joint scheduling and power control (near-optimal) \\};
	\end{tikzpicture}
	
	
	\caption{Fairness comparison of connectivity of a VUE ($\nTx=20,\,T=12,\nRx=20$)}	 \label{Fig:CDFandEachVUEPerformance}
\end{figure*}

\endgroup


